Rethinking Graph Regularization for Graph Neural Networks

The graph Laplacian regularization term is usually used in semi-supervised representation learning to provide graph structure information for a model $f(X)$. However, with the recent popularity of graph neural networks (GNNs), directly encoding graph structure $A$ into a model, i.e., $f(A, X)$, has become the more common approach. While we show that graph Laplacian regularization brings little-to-no benefit to existing GNNs, and propose a simple but non-trivial variant of graph Laplacian regularization, called Propagation-regularization (P-reg), to boost the performance of existing GNN models. We provide formal analyses to show that P-reg not only infuses extra information (that is not captured by the traditional graph Laplacian regularization) into GNNs, but also has the capacity equivalent to an infinite-depth graph convolutional network. We demonstrate that P-reg can effectively boost the performance of existing GNN models on both node-level and graph-level tasks across many different datasets.

==> 2_background.tex <==

\section{Background}
\subsection{Problem Definition}
Given a graph \(G = (V, E)\), where \(V\) denotes the set of \(N\) nodes, with features \(X \in \mathbb{R}^{N \times F}\) and one-hot labels \(Y \in \mathbb{R}^{N \times C}\) and the set of edges \(E\), can be denoted as adjacency matrix \(A \in \mathbb{R}^{N \times N}\). \(F\) and \(C\) are the dimensions of the node features and node labels, respectively.

Considering the semi-supervised node classification task for a graph \(G\), usually we have a small amount of nodes with labels, which can be treated as training nodes plus validation nodes. With the given graph topology \(A \in \mathbb{N}^{N \times N}\), node features \(X \in \mathbb{R}^{N \times F}\), and limited amount of labels \(Y_{seen} \in \mathbb{R}^{M \times C}\), where \(M\) is the total size of training set and validation set, we need to learn a model \(\mathcal{M}: \left(A, X, Y_{seen}\right) \rightarrow Y_{all}\), where \(Y_{all}\) is the labels for the whole graph \(G\).


\subsection{Traditional Laplacian Regularization Methods}

For the above classifying graph nodes problem, there are lots of previous work~\citep{zhu2003semi} adopting explicit regularization term to make use of the property of the smoothness of labels over the graph, that can be framed to 
\[
  \mathcal{L} = \mathcal{L}_{cls} + \mu \mathcal{L}_{reg},
\]

where the \(\mathcal{L}_{cls}\) is the supervised classification errors, and the \(\mathcal{L}_{reg}\) is the regularization term. \(\mu\) is the balance factor between \(\mathcal{L}_{cls}\) and \(\mathcal{L}_{reg}\). Common choices for the two loss terms are:
\[
  \begin{aligned}
  \mathcal{L}_{cls} &= \text{CrossEntropy}\left( \text{softmax}\left(f\left(X_{train}\right)\right) , Y_{train}\right), \\
  \mathcal{L}_{reg} &= \sum_{i,j}A_{ij}\left\|f(X_i) - f(X_j)\right\|_2^2 = \text{Tr}\left( f(X)^\top \Delta f(X)\right),
  \end{aligned}
\]
where the \(\Delta\) denotes the graph Laplacian matrix, which is \(\Delta = D - A\), and \(D\) is the diagonal matrix for nodes in the graph, \(D = \text{diag}(d_1, d_2, \ldots, d_N)\), where \(d_i\) denotes the degree of the \(i\)-th node. \(\text{Tr}\left(\cdot\right)\) denotes the \textit{trace} of the matrix. The \textit{CrossEntropy} function is defined over the predicted class posterior distribution \(P \in \mathbb{R}^C\):
\[
    \text{CrossEntropy}(P, Y_{train}) = \sum_{i \in S_\text{train}}\sum_{j \in \left[1,C\right]} - Y_{ij} \log\left(P_{ij}\right),
\]
where \(S_\text{train}\) is the set of indices of training nodes, and the predicted class posterior distribution \(P \in \mathbb{R}^{N \times C}\) is from the \textit{softmax} of the model outputs \(F=f(X) \in \mathbb{R}^{N \times C}\):
\[
    P_{ij} = \text{softmax}\left(F\right)_{ij} = \frac{\exp(F_{ij})}{\sum_{k=1,\ldots, C}\exp(F_{ik})} \quad \text{for } i = 1,\ldots, N \text{ and } j = 1 ,\ldots, C.
\]



\subsection{Graph Neural Network Methods}

Recently great advances in graph node classification task was introduced by a series of graph neural network models. GNN resolved the above limitation to some extent. Instead of modeling independently on the node features, i.e., \(f(X): \mathbb{R}^{N\times F} \rightarrow \mathbb{R}^{N \times C}\), graph neural network directly models the graph topology and node features at the same time, i.e., \(f(A, X): \left(\mathbb{N}^{N\times N}, \mathbb{R}^{N\times F}\right) \rightarrow \mathbb{R}^{N \times C}\). This makes the model have the ability to use the graph structure information inherently, resulting in much higher capacity. Thus the explicit regularization term can be eliminated, then the model can be trained only with the classification loss:
\[
  \mathcal{L} = \text{CrossEntropy}\left(\text{softmax}\left(f\left(A, X\right)\right), Y_{train}\right).
\]

Many popular and efficient graph neural network models are proposed. For example,  Graph Convolution Network~\citep{kipf2017semi} is defined as \(f_{GCN}(A, X) = \hat{A}(\text{ReLU}\left(\hat{A}XW_0\right))W_1\), where \(\hat{A}\) is the normalized adjacency matrix, could be \(\hat{A} = \tilde{D}^{-1}\tilde{A}\), and \(\tilde{A}=A+I\) is the graph with self-loop and \(\tilde{D}\) is the diagonal degree matrix of \(\tilde{A}\). Or we can also use the re-normalization trick, as \(\hat{A} = \tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}}\). Graph Attention Network~\citep{velickovic2018graph} brought the Attention mechanism to GCN , as \(f_{GAT}(A, X) = A'_1(\text{ReLU}\left(A'_0XW_0\right))W_1\), where \(A'_{ij} = \frac{\exp \left(\text { LeakyReLU }\left(\vec{a}^{T}\left[W \vec{h}_{i} \| W \vec{h}_{j}\right]\right)\right)}{\sum_{k \in \mathcal{N}_{i}} \exp \left(\text { LeakyReLU }\left(\vec{a}^{T}\left[W \vec{h}_{i} \| W \vec{h}_{k}\right]\right)\right)}\). Simplifying Graph Convolution Network~\citep{felix2019simplifying} is to demonstrate the non-linearity in GCN could be avoided, as \(f_{SGC}(A, X) = \hat{A}^KXW\), where \(K\) denotes the number of layers in SGC. 


